Who Goes First? Influences of Human-AI Workflow on Decision Making in Clinical Imaging

Details of the designs and mechanisms in support of human-AI collaboration must be considered in the real-world fielding of AI technologies. A critical aspect of interaction design for AI-assisted human decision making are policies about the display and sequencing of AI inferences within larger decision-making workflows. We have a poor understanding of the influences of making AI inferences available before versus after human review of a diagnostic task at hand. We explore the effects of providing AI assistance at the start of a diagnostic session in radiology versus after the radiologist has made a provisional decision. We conducted a user study where 19 veterinary radiologists identified radiographic findings present in patients' X-ray images, with the aid of an AI tool. We employed two workflow configurations to analyze (i) anchoring effects, (ii) human-AI team diagnostic performance and agreement, (iii) time spent and confidence in decision making, and (iv) perceived usefulness of the AI. We found that participants who are asked to register provisional responses in advance of reviewing AI inferences are less likely to agree with the AI regardless of whether the advice is accurate and, in instances of disagreement with the AI, are less likely to seek the second opinion of a colleague. These participants also reported the AI advice to be less useful. Surprisingly, requiring provisional decisions on cases in advance of the display of AI inferences did not lengthen the time participants spent on the task. The study provides generalizable and actionable insights for the deployment of clinical AI tools in human-in-the-loop systems and introduces a methodology for studying alternative designs for human-AI collaboration. We make our experimental platform available as open source to facilitate future research on the influence of alternate designs on human-AI workflows.

==> text/ideas.tex <==
  

Contributions: open-source platform, takeaways from experiment


% TODO: we should check whether these differences disappear in later stages!
% TODO: look at the stat analysis in the other AI in medicine papers. Should we
% go with hierarchical models, GEEs, or simply be agnostic about the correlation
% structure and use the mean (e.g., of time x participant)?
\begin{itemize}
\item On average, radiologists spent about 3 minutes on each diagnostic task
(median is about 2 and a half minutes). The time spent does not differ in a
significant way across the two workflows.  
\begin{itemize}
    \item The time spent largely varies across radiologists. For example, five
    of the radiologists solved each task in 2 minutes or less. By contrast, five
    other radiologists spent on average more than 5 minutes on each of these
    tasks. 
    \item Participants with previous RAI exposure (who also tend to have more
    years of experience) generally spend more time on the task. 
    \item The first tasks in the experiment took the participants the longest
    amount of time, compared to the remaining tasks.
\end{itemize}
\item Agreement between the RAI's and radiologists' diagnoses is higher in the
1-step workflow, regardless of whether the RAI's diagnosis is correct. This
indicates the presence of {\emph anchoring effects}. However, agreement largely
varies across participants.
% it might have been a good idea to do a within-subjects design with the washout
% period
\begin{itemize}
    \item 
\end{itemize}
\item despite the presence of anchoring, we could not detect
sizeable differererences in predictive accuracy and consistency (due to the low base rate)
% TODO: should recheck this part conditioning on the positives
\item second opinions increase when the AI is presented directly
\end{itemize}

==> text/notes.tex <==



% TODO comment on the fact that radiologists waste time looking at images that
% are really not present

\subsection{Anchoring effects}

The final diagnoses provided by the participants matched the AI's binary
estimates in 91\% and 89\% of the cases in the one-step workflow and two-step
workflows respectively. When the condition was flagged by the AI, participants
in the one-step workflow diagnosed it as being present more often than their
counterparts (71\% and 65\% of the cases respectively). However, higher reliance
was not always warranted: Presenting the AI directly led to more agreement both
when recommendations were correct () but also when they were inaccurate ().

% choose one of the following
% this does not really enter here
The effect of the workflow configurations is most salient for cases
characterized by high diagnostic uncertainty. 
% TODO: revise
% As a first example, consider the  
% conditions for which AI confidence was between 0.4 and 0.8. 
If participants'
judgment had been affected by the AI's binary recommendations, we would expect
such an impact to be largest for the diagnoses made in the one-step workflow. 
% When the condition was flagged by the AI (i.e.,
% confidence $\geq$0.6), 54\% and 45\% of the diagnoses made participants in the
% one- and two-step workflows respectively matched the recommendation. When the
% condition was not flagged, 15\$ and 18\% of the conditions respectively were
% diagnosed as being present. 
% TODO: switch to RD figure
In Figure XX, we employ a regression discontinuity design to analyze the
association between AI's recommendations and participants' diagnoses. We observe
that, controlling for AI confidence, the AI flagging the condition (i.e.,
confidence$\geq$60\%) led to a sizeable jump in the likelihood that participants
assigned to the one-step workflow will diagnose the condition as present. This,
however, does not occur for those in the two-step workflow. A nonparametric analysis
further corroborates this difference: \dots 

% not very convincing - drop because when radiologists believe that a condition
% is there there is large disagreement
As a second example, consider the set of conditions for which only 50\%--60\% of
the diagnoses provided by the pool of radiologists prior to our experiment
matched, i.e., there was substantial disagreement. When the condition was
flagged by the AI, participants diagnosed it as present in 83\% and 75\% of the
cases in the one- and two-step workflows. When the condition was not flagged,
the shares of these diagnoses dropped to 59\% and 68\% respectively.  

% discuss critical and non critical conditions
We find that participants in the one-step workflow agreed with the AI binary
recommendations across almost all of the conditions. The gap in the level of
agreement between the two workflows was highest for the non-critical conditions \dots


% discuss how often people change opinions
We can also look at how the AI influenced participants' judgment ... Even before
receiving the AI's advice, 88\% of the diagnoses made by participants in the
two-step workflow matched the AI's. This is only marginally lower than the level
of agreement for their final diagnoses (89\%). Indeed, these participants
revised their diagnoses for only 5\% of the conditions where the AI's
recommendation did not match their initial decision. Among the cases where there
was initial disagreement between AI and participants, the revision occured more
frequently when the AI had flagged a condition that had not initially been found
by the participant (10\% of these diagnoses were revised). 
% This means that participants diagnosed more conditions as present after seeing the AI's advice. 
The revisions mainly concerned conditions that \dots [TODO: add analysis by
condition based on Diane's feedback]


The observed anchoring effect has several consequences. First, it reduces
inter-rater variability: Fleiss' kappas were 0.55 and 0.49 for the diagnoses
made with AI assistance in the one- and two-step workflows respectively. 

% not really sure about predictive performance

 
\subsection{Effort and time spent on decision-making}
% time, utility, mental effort, and confidence

Ex ante we expected that revealing the AI recommendations only after
participants had made an initial diagnosis would substantially slow down their
decision-making process. However, we found no significant differences across the
two workflows in terms of the average and median time (3 and 2 and 1/2 minutes
respectively) spent reviewing the images. To explain this null finding, we can
build off of the results of our previous analysis.  
We have seen that participants assigned to the two-step workflow rarely changed
their initial diagnoses or asked for a second opinion after seeing the AI's
recommendations, even in cases of disagreement. Consistently with this finding,
we observe that these participants spent only one fourth of their. In addition,
images where the AI flagged a larger share of the conditions took proportionally
more time to participants in the two-step workflow compared to their
counterparts. These results would suggest that participants who were shown
directly the AI advice might have spent more time second guessing their
diagnoses.
% TODO: think again about this. How can we explore this direction further?


Despite spending similar time on the review of the image, participants in the
two-step workflow found the task to be more stressful and demanding than those
in the one-step workflow (aggregate mean scores on Likert scale 1--7 were 3.8
and 4.4 respectively). 

After reviewing each image, participants were asked whether the AI
recommendation had been useful or not. Participants assigned to the one- and
two-step workflow reported that the AI advice was useful in 36\% and 17\% of the
cases. In the questionnaire administered at the end of the second stage, we
asked participants to dinsentangle the utility (or lack thereof) in terms of
gains in accuracy, speed, and confidence in the diagnoses. Those in the two-step
workflow gave again substantially lower ratings across all three dimensions,
especially with respect to speed for which the mean scores were 4.2 and 2.5 on
Likert scale 1--7 resspectively. Even after controlling for the opinions
collected in our initial survey, the gap in the ratings relative confidence
still persist.
% do we have a question about speed in that survey?
% why is it the case that participants feel that it is less useful?
These participants also reported being less willing to use the AI tool in their
jobs in the future. 




\subsection{Seeking second opinions}

% second opinions
For each diagnosis, participants were asked whether, were they to encounter the
same case in their daily jobs, they would seek the opinion of a colleague before
making the final call. Participants rarely indicated this option and there was
no substantial difference across the two workflows. On the one hand,
participants in the one-step workflow required second opinions more often than
those in the one-step workflow when they disagreed with the AI's
recommendations. For conditions that were not flagged by the AI but participants
diagnosed as present, the shares of second opinions sought in the one- and
two-step workflows were 11\% and 6\% respectively. When the condition was
flagged by the AI but participants did not believe it was present, the
respective shares were 2\% and 1\%. On the other hand, those in the two-step
workflow sought second opinions more often when they agreed with the AI that the
condition was present. In most of these cases, participants sought the second
opinion before seeing the AI and did not change their preference after receiving
the advice. Thus, they simply did not revise their answer to this question. In
the few cases for which these partcipants revised their initial diagnosis, they
often sought second opinions (14\% of all cases and 26\% of those not flagged by
the AI). 










